Formal Analysis of Quantum Systems using Process Calculus

Quantum communication and cryptographic protocols are well on the way to becoming an important practical technology. Although a large amount of successful research has been done on proving their correctness, most of this work does not make use of familiar techniques from formal methods, such as formal logics for specification, formal modelling languages, separation of levels of abstraction, and compositional analysis. We argue that these techniques will be necessary for the analysis of large-scale systems that combine quantum and classical components, and summarize the results of initial investigation using behavioural equivalence in process calculus. This paper is a summary of Simon Gay's invited talk at ICE'11.

==> eptcsdata.tex <==
\providecommand{\firstpage}{104}
\providecommand{\publicationstatus}{Bliudze, S., Bruni, R., Carbone, M., Silva, A. (Eds.); ICE 2011\\
EPTCS 59, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.59.9}{10.4204/EPTCS.59.9}}

